AdaFPP: Adapt-Focused Bi-Propagating Prototype Learning for Panoramic Activity Recognition

Panoramic Activity Recognition (PAR) aims to identify multi-granularity behaviors performed by multiple persons in panoramic scenes, including individual activities, group activities, and global activities. Previous methods 1) heavily rely on manually annotated detection boxes in training and inference, hindering further practical deployment; or 2) directly employ normal detectors to detect multiple persons with varying size and spatial occlusion in panoramic scenes, blocking the performance gain of PAR. To this end, we consider learning a detector adapting varying-size occluded persons, which is optimized along with the recognition module in the all-in-one framework. Therefore, we propose a novel Adapt-Focused bi-Propagating Prototype learning (AdaFPP) framework to jointly recognize individual, group, and global activities in panoramic activity scenes by learning an adapt-focused detector and multi-granularity prototypes as the pretext tasks in an end-to-end way. Specifically, to accommodate the varying sizes and spatial occlusion of multiple persons in crowed panoramic scenes, we introduce a panoramic adapt-focuser, achieving the size-adapting detection of individuals by comprehensively selecting and performing fine-grained detections on object-dense sub-regions identified through original detections. In addition, to mitigate information loss due to inaccurate individual localizations, we introduce a bi-propagation prototyper that promotes closed-loop interaction and informative consistency across different granularities by facilitating bidirectional information propagation among the individual, group, and global levels. Extensive experiments demonstrate the significant performance of AdaFPP and emphasize its powerful applicability for PAR.

==> imgs/module.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/module-v3.pdf}% use pdf
    \caption{\textbf{Illustration of Bi-Propagating Prototype Learning.}}
    \label{fig3}
\end{figure}

==> imgs/motivation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/motivation_v5.pdf}% use pdf

    \caption{\textbf{Comparison between existing works and our proposed approach. a) The traditional method works on specific multi-granularity behaviour recognition in panoramic scenes, where individual feature extraction is performed using manually bounding boxes, followed by hierarchical modelling at three granularities: individual, social group and global during training and inference. b) Recent methods remain consistent with traditional methods during training, but add additional detectors for individual detection during inference to adapt to real panoramic scenes.
    c) Our proposed approach builds a joint framework for both individual detection and behaviour recognition, where we jointly train a panoramic person-focusing module and a multi-granularity behaviour recognition module, allowing for individual localization and action prediction during inference.}}
    \label{fig1}
\end{figure}

==> imgs/overview.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/Fig2_3.pdf}% use pdf
    \caption{\textbf{The overall Framework of Adapt-Focused Bi-Propagating Prototype Learning, which consists of two crucial modules, i.e., panoramic adapt-focuser and bi-propagating prototyper. The proposed framework aims to jointly recognize individual actions, social-group and global activities in panoramic activity scenarios by learning an adapt-focused detector and multi-granularity prototypes. The adapt-focuser is built to comprehensively localize individuals in panoramic images by adaptively selecting and performing detailed detection on object-dense subregions identified through coarse detections. Following this, the bi-propagating prototyper module utilizes the obtained individual localization to promote closed-loop interaction and informative consistency
    across different granularities by facilitating bidirectional information propagation from individual to social-group to global levels. Finally, the summation of detection and classification loss is used for the optimization of the
    whole model.}}
    \label{fig2}
\end{figure*}
